Demystifying Core Ranking in Pinterest Image Search

Pinterest Image Search Engine helps hundreds of millions of users discover interesting content everyday. This motivates us to improve the image search quality by evolving our ranking techniques. In this work, we share how we practically design and deploy various ranking pipelines into Pinterest image search ecosystem. Specifically, we focus on introducing our novel research and study on three aspects: training data, user/image featurization and ranking models. Extensive offline and online studies compared the performance of different models and demonstrated the efficiency and effectiveness of our final launched ranking models.

==> sec-overview.tex <==
\section{Architecture Overview}
Figure~\ref{fig:system} depicts the overview of the Pinterest Image Search Architecture, which is essential to help understand why and how our system works. Whenever a user initiates a query, it goes through query processing steps. After that candidate pins are retrieved from different indexed corpora based on the processed query and attributes of the user. The core ranking and re-ranker component subsequently determines the importance of each candidate pin and provide the final impression to the client. Each system component and the sequence of events handled in them from the foremost user request to the ultimate impression are highlighted as follow:
\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{overview}
\caption{An Overview of Pinterest Image Search System}\label{fig:system}
\end{figure}

\begin{description}
\item[User Signal] In this component, we build and leverage profiles of users to improve the quality of image search. Specifically, we maintain the gender, country and locale information of users as well as intents of users. 
\item[Query Processing] In search engine, keyword research is the beginning of the journey. It's our best bet to understanding what people are searching for. Our query processing components consists of standard text pre-processing(such as tokenization, stemming), auto-completion, spell correction, query expansion, query translation, query rewrite, search guides and query intent understanding.
\item[Indexing and Candidate Generation] Our in-house Manas\footnote{https://medium.com/@Pinterest\_Engineering/manas-a-high-performing-customized-search-system-cf189f6ca40f} System supports finding the most relevant results among +100 billion Pins for every Pinner through indexing and candidate generation. 
\item[Core Ranking] Learning to rank or machine-learned ranking (\texttt{MLR}) is one of the most central components in any search engine. Like other common \texttt{MLR} components, we featurize user, query, and image signals into feature vectors, and then apply learning algorithms to obtain the quality score of each image to generate the final ordering of impression. In order to strike the balance between efficiency and effectiveness, while to improve the diversity and freshness of content, in our core ranking component, we also design and develop a cascading ranking pipeline that consists of three stages: lightweight ranking stage, full ranking stage, and re-ranking stage.
\end{description}

In this work, we focus on sharing our experiences in tackling the search quality issues and introduce a series of practical techniques that have been successfully launched to power the Pinterest image search engine. Specifically, we present how we help users discover high-quality images with our cascading core ranking in Section~\ref{sec:ranking}.









